Learning High-DOF Reaching-and-Grasping via Dynamic Representation of Gripper-Object Interaction

We approach the problem of high-DOF reaching-and-grasping via learning joint planning of grasp and motion with deep reinforcement learning. To resolve the sample efficiency issue in learning the high-dimensional and complex control of dexterous grasping, we propose an effective representation of grasping state characterizing the spatial interaction between the gripper and the target object. To represent gripper-object interaction, we adopt Interaction Bisector Surface (IBS) which is the Voronoi diagram between two close by 3D geometric objects and has been successfully applied in characterizing spatial relations between 3D objects. We found that IBS is surprisingly effective as a state representation since it well informs the fine-grained control of each finger with spatial relation against the target object. This novel grasp representation, together with several technical contributions including a fast IBS approximation, a novel vector-based reward and an effective training strategy, facilitate learning a strong control model of high-DOF grasping with good sample efficiency, dynamic adaptability, and cross-category generality. Experiments show that it generates high-quality dexterous grasp for complex shapes with smooth grasping motions.

==> figures/ablation_studies.tex <==
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.96\linewidth]{images/demonstration.pdf}
	\includegraphics[width=0.96\linewidth]{images/demonstration.pdf}
	\includegraphics[width=0.96\linewidth]{images/demonstration.pdf}
	\caption{Visual comparisons of results obtained with different settings of our methods. }
	\label{fig:ablation_studies}
\end{figure}


==> figures/diff_shape.tex <==
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.96\linewidth]{images/diff_shape.pdf}
	\caption{Example results where we fix the initial gripper configuration and plan the grasping for different 3D shapes.  }
	\label{fig:diff_shape}
\end{figure}


==> figures/init_position.tex <==
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.96\linewidth]{images/init_position.pdf}
	\caption{A sampling of initial gripper configuration on the hemisphere determined by the object center. For all the initial configurations, the palm is facing toward the object center.  We show two example initial configurations on the left and points on the hemisphere that correspond to the fixed setting set of initial configurations on the right.	}
	\label{fig:init_position}
\end{figure}


==> figures/tab_comp_baseline.tex <==
\begin{table}[!t]%
	\caption{Comparison to the baseline~\cite{liu2020deep} considering the final grasping only.
		The measures are the average generalized $Q_1$, the average standard $Q_1$, the average non-zero penetration ($mm$), the Success-Grasp-Rate based on generalized $Q_1$, and the Success-Grasp-Rate based on standard $Q_1$. }
	\label{tab:comp_baseline}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{l||l|l|l|l|l}
				\hline\hline
				\textbf{Method} &   $Q_1^g$ & $Q_1^s$&  $P $  &  $R_{\text{grasp}}^g$  & $R_{\text{grasp}}^s$   \\ \hline \hline
				\cite{liu2020deep} & 0.187 & 0.284 & 9.41  & 90.07$\%$ & 36.17$\%$ \\  \hline
				Ours (TOP-1) & 0.217  & 0.242 &  1.26   &  95.04$\%$ &  83.69$\%$ \\  \hline
				Ours (TOP-5) & 0.186  & 0.130 &  1.76  &  94.18$\%$  &  55.74$\%$ \\  \hline
				Ours (ALL) & 0.194 & 0.213 &  2.75  & 85.86$\%$  &  38.30$\%$  \\ \hline \hline
			\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%

